Learning Native Reflection in Unified Models with Interleaved Reinforcement Learning

Unified multimodal models can both look at and render images, so in principle they can repair their own generations: diagnose what an image gets wrong, revise it, observe the result, and diagnose again. Whether a revision helps is known only after it is rendered, so the reflection text and the image generation must be learned jointly, over the whole loop. Supervised fine-tuning (SFT) on reflection trajectories gives a cold start but does not find the high-success repair paths, and naive RL that optimizes only the renderer or only one head leaves most of the gain untapped. We introduce UMM-Reflection, which applies reinforcement learning (RL) to complete reflection trajectories inside one unified model: sibling trajectories share one initial image, so the group-relative advantage compares reflection strategies, and one trajectory-level advantage updates both the reflection tokens and the flow-based revisions, avoiding the combinatorial blow-up of per-round credit assignment. Unlike single-round editing or pipelines with an external critic, credit flows across rounds and to both roles of the same model, and no verifier is needed at inference. On BAGEL, UMM-Reflection improves GenEval by 12.05 points over SFT, and the gains transfer to WISE (+10.97), OneIG-Bench (+3.48), and T2I-CompBench++ (+4.63), none of which is used in training.

==> tables/compbench_results.tex <==
\begin{tabular}{lrrr}
\toprule
Category & BAGEL & RL initial & RL final \\
\midrule
Color & 74.37 & 72.32 & 84.02 \\
Shape & 52.16 & 51.82 & 62.24 \\
Texture & 66.58 & 67.82 & 75.66 \\
Non Spatial & 30.79 & 30.85 & 30.65 \\
Spatial & 30.15 & 31.19 & 40.77 \\
3D Spatial & 39.13 & 38.22 & 36.72 \\
Numeracy & 60.67 & 60.10 & 64.48 \\
Complex & 38.47 & 38.30 & 40.52 \\
\bottomrule
\end{tabular}


==> tables/dev_results.tex <==
\begin{tabular}{lrrrr}
\toprule
Model & Initial & Final & Repair & Damage \\
\midrule
Reflection SFT & 64.4 & 66.3 & 15.6 & 5.7 \\
\method{} (100 updates) & 63.7 & 69.3 & 28.6 & 7.6 \\
\method{} (200 updates) & 64.4 & 70.4 & 31.2 & 8.0 \\
\bottomrule
\end{tabular}


==> tables/published_results.tex <==
\begin{tabular}{lrl}
\toprule
Model & Native GenEval & Original source \\
\midrule
Emu3-Gen & 0.54 & \citet{emu32024}, Table 7 \\
TokenFlow & 0.55 & \citet{tokenflow2024}, Table 10 \\
ILLUME & 0.61 & \citet{illume2024}, Table 4 \\
Janus & 0.61 & \citet{janus2024}, Table 3 \\
Show-o-512 & 0.68 & \citet{showo2024}, Table 3 \\
Janus-Pro-7B & 0.80 & \citet{januspro2025}, Table 4 \\
\bottomrule
\end{tabular}


==> tables/round_scaling.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
 & \multicolumn{5}{c}{Accuracy by budget} & \multicolumn{3}{c}{Reflection} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-9}
Model & R0 & +1 & +2 & +3 & $\Delta$ & Repair & Damage & Edits \\
\midrule
Base & 71 & 72 & 73 & 73 & +1 & 17.8 & 5.9 & 1.25 \\
SFT & 70 & 71 & 72 & 72 & +2 & 20.6 & 6.5 & 1.65 \\
\midrule
RL ckpt\,100 & 71 & 74 & 75 & 75 & +3 & 35.6 & 9.5 & 3.00 \\
RL ckpt\,200 & 72 & 76 & 76 & 79 & +7 & 44.1 & 7.7 & 2.99 \\
RL ckpt\,300 & 72 & 80 & 83 & 81 & +9 & 56.0 & 9.1 & 3.00 \\
RL ckpt\,400 & 72 & 79 & 80 & 82 & +10 & 60.4 & 10.4 & 2.98 \\
RL ckpt\,500 & 71 & 75 & 82 & 82 & +11 & 61.1 & 9.3 & 3.00 \\
\rowcolor{bakerlrow}RL ckpt\,1000 & 73 & 82 & 84 & 84 & +11 & 64.9 & 8.8 & 3.00 \\
\bottomrule
\end{tabular}


==> tables/stopping_variant.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Checkpoint & R0 & +1 & +2 & +3 & Repair & Damage & Edits & Stopped early \\
\midrule
200 & 72 & 76 & 76 & 76 & 39.4 & 9.4 & 1.20 & 97.6\% \\
400 & 70 & 78 & 81 & 81 & 61.4 & 11.0 & 1.22 & 94.9\% \\
500 & 62 & 78 & 79 & 79 & 61.1 & 9.5 & 1.08 & 98.2\% \\
\bottomrule
\end{tabular}


==> tables/t2i_rl_ablation.tex <==
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
Model & Parent & RL steps & Repairs & GenEval & WISE & OneIG & T2I-CompBench++ \\
\midrule
BAGEL-Base & Base & 0 & 0 & 71 & 55 & 80 & 49 \\
BAGEL-T2I-RL & Base & 1000 & 0 & 76 & 54 & 80 & 49 \\
BAGEL-SFT & SFT & 0 & 3 & 72 & 63 & 79 & 50 \\
\rowcolor{bakerlrow}\method{} (final) & SFT & 1000 & 3 & \textbf{84} & \textbf{74} & \textbf{83} & \textbf{55} \\
\bottomrule
\end{tabular}


==> tables/understanding_bestof4.tex <==
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
Method & Single & Two & Count & Colors & Position & Binding & Overall \\
\midrule
\multicolumn{8}{l}{\textit{Local evaluation: same prompts, resolution, and scorer}} \\
BAGEL-Base & \textbf{1.00} & 0.89 & 0.63 & 0.82 & 0.47 & 0.48 & 0.71 \\
Base Bo4 + Base UND & \textbf{1.00} & 0.93 & \textbf{0.74} & 0.85 & 0.59 & 0.58 & 0.78 \\
\rowcolor{bakerlrow}\method{} & 0.95 & \textbf{0.96} & 0.68 & \textbf{0.90} & \textbf{0.89} & \textbf{0.65} & \textbf{0.84} \\
\bottomrule
\end{tabular}

